Scaling Deep Contrastive Learning Batch Size under Memory Limited Setup

Contrastive learning has been applied successfully to learn vector representations of text. Previous research demonstrated that learning high-quality representations benefits from batch-wise contrastive loss with a large number of negatives. In practice, the technique of in-batch negative is used, where for each example in a batch, other batch examples' positives will be taken as its negatives, avoiding encoding extra negatives. This, however, still conditions each example's loss on all batch examples and requires fitting the entire large batch into GPU memory. This paper introduces a gradient caching technique that decouples backpropagation between contrastive loss and the encoder, removing encoder backward pass data dependency along the batch dimension. As a result, gradients can be computed for one subset of the batch at a time, leading to almost constant memory usage.

==> impact.tex <==
\section{Broader Impact}

Today's use of cloud computing offers the flexibility to scale up hardware to a certain extent. When possible, higher-capacity hardware offers the most effective way of scaling training batch size.
However, when a set of hardware is already built, it could take non-trivial efforts to grow further. Our technique enables scaling batch size for contrastive learning far beyond the limitation of GPU memory. With it, researchers can validate ideas without waiting for hardware updates and push the research boundary of large batch training, designing better models, objectives, and optimizers.

More importantly, we observe that for many university research groups (and small startup companies), the use of consumer-grade hardware usually caps the deep learning machine at 4 GPU systems with roughly 40G of GPU memory in total. In comparison, the popular DGX workstation in the industry offers 8 cards with about 240G of GPU memory, not to mention the cloud TPUs at Google. Our technique removes the memory limitation and alleviates the hardware gap. It allows experiments to be conducted at a larger scale under an academic setup: in particular, university researchers can replicate experiments done with higher capacity hardware. Meanwhile, adaptations of a pre-trained model for task and/or domain transfer does not need to compromise in batch size. In general, we make it possible for more people to work on and contribute to the problem and the application of contrastive learning.

The results of the scaling test show that merging batches with our methods can lower total computation time by reducing the number of optimizer steps. With optimization techniques~\cite{LARS,LAMB} that can use a large batch to produce an equal or better result with \emph{equal or less} data than a small batch, our method provides a means to reduce the total computation time for limited resource learning.
